Formation of sediment patterns in channel flow: minimal unstable systems and their temporal evolution

The phenomenon of sediment pattern formation in a channel flow is numerically investigated by performing simulations which resolve all the relevant scales of the problem. The numerical approach employed and the flow configuration considered is identical to our previous study (Kidanemariam and Uhlmann J. Fluid Mech., vol. 750, 2014, R2), the only difference being the length of the computational domain. By successively reducing the streamwise length, the minimum box dimension which accommodates an unstable sediment bed is revealed, thus determining the lower threshold of the unstable modes. For the considered parameter point, the cutoff length for pattern formation lies in the range 75-100 particle diameters (3-4 times the clear fluid height). We also simulate the flow in a very long streamwise box with a size of 48 times the clear fluid height (featuring over one million particles), accommodating approximately 11 initial ripple units with a wavelength of 100-110 particle diameters. The amplitude of the patterns exhibits two regimes of growth: an initial exponential regime, with a growth rate independent of the chosen domain size, and a subsequent non-linear regime which is strongly constrained by the domain length. In the small domain cases, after the initial exponential regime, the ripples evolve steadily maintaining their shape and migration velocity, at a mean wavelength equal to the length of the domain. The asymmetric ripple shape is characterized by a spectrum which exhibits a power-law decay over the first few dominant non-dispersive modes propagating at the mean dune migration velocity. The particle flowrate and the mean interface shear stress exhibited an increase with increasing ripple dimensions. Nevertheless, the relationship between the two was observed to be approximately described by the empirical power law formula for sediment transport by Wong & Parker (2006).

==> friction_velocity.tex <==
%
\section{Determination of friction velocity}
\label{sec:friction-velocity}
%
\comment{under construction}

As was mentioned in section~\ref{sec:setup}, the pressure 
gradient which
drives the flow is adjusted at each time step in order to maintain a 
constant flow rate. Thus the value of the pressure gradient is not known
{\it a priori}. However, 
%
the instantaneous value of the pressure gradient can be determined
%
from the balance between the driving volume force
(resulting from the imposed pressure gradient itself) and resisting forces,
taking into account the incompressibility constraint.
As a result of the free-slip boundary condition at the top of the domain,
the resistance is entirely due to the total hydrodynamic and inter-particle
collision forces exerted by the stationary particles located beneath the
mobile sediment layer upon the fluid and mobile particles. 
The contribution from the shear stress at the
bottom smooth wall beneath the stationary particles is negligibly small due
to the almost zero velocity gradients therein. Thus,
%
\begin{equation}\label{eq:flwpatt-dpdx-vs-particle-forces}
        \dpdx(t) = %
                    -\frac{1}{\Lx\Ly\Lz}\sum_{l=1}^{N_p}
                    \Big(
                        F^{H(l)}_{p,x}(t)+F^{C(l)}_{p,x}(t)
                    \Big)I_{stat}^{(l)}\;,
\end{equation}
%
where $F^{H(l)}_{p,x}$ and $F^{C(l)}_{p,x}$ are the streamwise component of 
the hydrodynamic and collision forces acting upon the $l$th particle,
respectively. $I_{stat}^{(l)}$ is an indicator function which has a value 
of unity if the $l$th particle is stationary and zero otherwise.

Moreover, in a fully-developed particle-laden channel flow, the mean 
pressure gradient is slope of the wall-normal profile of the total shear 
stress, where the latter
is the sum of viscous shear stress, Reynolds shear stress and stress 
contribution from the fluid-particle interaction 
\citep{Uhlmann2008,Kidanemariam2013}. Thus,  \dpdxmeanline\
is related to the bottom wall friction as 
%
\begin{equation}\label{eq:dpdx-vs-bottom-friction}
        \dpdx(t) = %
                    -\frac{\rhof u_*^2(t)}{\hfluid(t)}\;.
\end{equation}
%
where $u_*$ is a spatially averaged instantaneous friction velocity.
In the configurations considered in this study however, due to the roughness 
introduced as a result of the evolving sediment bed, a  
`horizontal bottom wall' does not exist. Nevertheless, a virtual wall 
could be defined to be located at a wall-normal location of 
$y=\hbed(t)$. A spatially-averaged instantaneous bottom friction
(thus friction velocity) is then computed from 
(\ref{eq:flwpatt-dpdx-vs-particle-forces}) and 
(\ref{eq:dpdx-vs-bottom-friction}). Alternatively, the instantaneous 
bottom friction could also be determined by extrapolating a linear line, 
which is fitted to the total shear stress profile in the clear fluid region, 
down  $y=\hbed(t)$. 
%
We opted for the former approach due to the precise determination of the 
instantaneous pressure gradient from our DNS data.

